A Data-Efficient Visual-Audio Representation with Intuitive Fine-tuning for Voice-Controlled Robots

A command-following robot that serves people in everyday life must continually improve itself in deployment domains with minimal help from its end users, instead of engineers. Previous methods are either difficult to continuously improve after the deployment or require a large number of new labels during fine-tuning. Motivated by (self-)supervised contrastive learning, we propose a novel representation that generates an intrinsic reward function for command-following robot tasks by associating images with sound commands. After the robot is deployed in a new domain, the representation can be updated intuitively and data-efficiently by non-experts without any hand-crafted reward functions. We demonstrate our approach on various sound types and robotic tasks, including navigation and manipulation with raw sensor inputs. In simulated and real-world experiments, we show that our system can continually self-improve in previously unseen scenarios given fewer new labeled data, while still achieving better performance over previous methods.

==> Sections/01-Introduction.tex <==
\section{Introduction}
\label{sec:intro}
% As robots begin to enter people's daily lives, there is an increasing need for mechanisms that allow non-experts to interact and communicate with robots in an intuitive way. 
As robots begin to enter people's daily lives, there is an increasing need for non-experts to intuitively interact and communicate with robots, which leads to a wealth of research in voice-controlled robots~\cite{liu2019review}. Conventional voice-controlled robot consists of independent modules for automatic speech recognition (ASR), natural language understanding (NLU), symbol grounding, and motion planning (Fig.~\ref{fig:diff_model}a). However, this design suffers from intermediate and cascading errors among different modules and the difficulties in grounding language to the physical entities~\cite{tada2020robust}.
%To address these challenges, several approaches attempt to jointly optimize some of the independent modules~\cite{serdyuk2018towards,hermann2017grounded}. However, these approaches only consider part of the pipeline and cannot solve voice-controlled tasks alone. 
The first end-to-end model for task-oriented voice-controlled robots and Robot Sound Interpretation (RSI) is proposed in~\cite{chang2020robot} to resolve the problems of the modular design. The RSI agent learns from raw image and audio signals and can learn the meaning of all types of sound in addition to speech. For example, an RSI agent is able to open a door when it hears either a person saying "open the door" or the chimes from the doorbell.
% This property, for example, allows the agent to open the door when either a speech command or the chimes from the doorbell are heard.
%Agents can learn language better when the language is presented and interpreted in the context of the world it pertains to~\cite{matuszek2018grounded}. 

RSI considers different robotic tasks in various settings as illustrated in Fig.~\ref{fig:opening}. given a sound command, the robot must identify the commander's goal (intent), draw the correspondence between the raw visual and audio inputs, and develop a policy to finish the task. The tasks are challenging because the observation mainly comes from a monocular uncalibrated RGB camera. No maps, depth images, human demonstrations, or prior knowledge is available.
% For example, in the Kuka environment, the agent learns to move by observing the pose of its gripper tip and the blocks from RGB images without relying on the object appearance. In the iTHOR environment, the agent needs to perform challenging mapless navigation to fulfill real multi-word speech commands.~\cite{tai2017virtual, partsey2022mapping}.
% Talk about the difficulty

    %The robots must approach a target mentioned by a sound command to finish a task. 
   
    


The model in~\cite{chang2020robot} directly maps sound commands and image observations to a sequence of robot actions that fulfill the commands, as illustrated in Fig.~\ref{fig:diff_model}b. The model is first trained in a simulated environment using reinforcement learning (RL) and auxiliary losses, and then the model is deployed to a real robot without further training.  

However, this method has its own weaknesses. 
% First, the design choices for the reward function limit the generalization of the method. The reward functions need to be hand-tuned and are task-specific, and thus cannot be used across different tasks or robotic platforms. 
First, the reward functions need to be hand-tuned and are task-specific, which limits the generalization of the method.
Second, it is costly to fine-tune the system in a new domain. Ideally, when an intelligent voice-controlled robot encounters unseen scenarios such as new speakers or new room layouts, it should continually improve its interpretation of language and skills from non-experts in daily life. However, similar to most learning-based systems, the performance of the model degrades due to domain shift~\cite{james2019sim,akkaya2019solving,Tobin_2017}. Improving the system in the new domain requires accurate measurements to calculate the reward and prohibitive amount of one-hot labels for image and sound classification, both of which are hard to obtain from and not intuitive to non-experts.
% Finally, the trained representation of sounds and images cannot be reused in other settings because of the end-to-end training of the representations and robotic tasks. 

Based on the recent advancements in representation learning, we address these weaknesses in~\cite{chang2020robot} by proposing a two-stage pipeline for training RSI agents as shown in Fig.~\ref{fig:diff_model}c. At the first stage, we train a visual-audio representation (VAR) using paired data that can be collected easily and intuitively by non-experts.
% At the second stage, we use the VAR to facilitate RL training. The VAR produces an intrinsic reward function that is general across tasks or robotic platforms, which avoids the laborious reward engineering. 
At the second stage, we use the VAR to produce an intrinsic reward function for RL training. The intrinsic reward function is general across tasks or robots, which helps avoid the laborious reward engineering.
% After the robot is deployed in a new domain where an accurate reward is hard to obtain or not available, non-experts can easily improve the VAR with a reasonable amount of training data, which allows the robot to perform self-supervised skill improvement using the updated intrinsic reward function. 
After the robot is deployed in the real world, non-experts can collect a reasonable amount of new data intuitively and update the VAR and the intrinsic reward without providing speech transcriptions, class labels, or tuned reward functions. The robot can then perform self-supervised skill improvement. 
% non-experts can provide a reasonable amount of training data to the system, which updates the intrinsic reward function from the VAR and allows the robot to perform self-supervised skill improvement. 

\begin{figure}[t]
    \centering
    \vspace{5pt}
    \includegraphics[scale=0.65]{Figures/diffModel_short.png}
    \caption{\textbf{Illustration of different models for voice-controlled robots.} (a) A usual pipeline for voice-controlled robots.  Independent modules process the inputs. End-to-end SLU combines the ASR and the NLU, while end-to-end grounding combines the NLU and the grounding module. (b) The first RSI model~\cite{chang2020robot}. Auxiliary losses such as $\mathcal{L}_{I}$ and $\mathcal{L}_{S}$ are used for classifying images and the intent in the speech, respectively. The model is trained end-to-end with an RL loss, $\mathcal{L}_{RL}$. (c) The proposed model. The intrinsic reward is denoted by $r^i$.}
    \label{fig:diff_model}
    \vspace{-20pt}
\end{figure}

% To show the applications of our method, we create the first AI environment that uses real multi-word speech commands for instruction-following tasks. We use AI2THOR~\cite{ai2thor}, a visually high-fidelity interactive simulator, and the Fluent Speech Commands (FSC)~\cite{lugosch2019speech} to build the environment. FSC is the state-of-the-art speech dataset collected for contemporary end-to-end spoken language understanding (SLU) system and contains free-form utterances from various speakers. 

%The method needs to be general in terms of sounds, robots, and tasks.
%We believe that every sound conveys meaning and can be used as a command to trigger robot actions. For this reason, the audio input includes not only speech but also musical tone and environmental sound. Besides,  




%  For example, infants can learn to associate an object with its name when they see the object and hear their parents say the name of the object immediately afterwards.

%Our method is inspired by sensorimotor contingency which is the relations between an agent's actions and the resulting sensory changes~\cite{o2011red}. Imagine that an infant touches a bell by accident and hears a bell ring. Motivated by her “intrinsic curiosity,” she attempts to replicate the sound by repeating and refining the touching action~\cite{jacquey2019sensorimotor}. When she hears a bell ring later, she should identify what actions are needed to ring the bell. 
%We believe that a robot can associate the motor actions with the corresponding audio command through a similar learning process. 
%Once the robot has developed sensorimotor contingencies from its previous embodied experiences, we can use a sound command to ask the robot to reach the goal and fulfill our intent. 
%The ability to relate language to the physical entities of the world allows the robot to communicate with humans on a mutual understanding, which leads to much more meaningful human-robot interactions~\cite{clark1991grounding, bisk2020experience}.

Our main contributions are as follows. (1) We present a novel voice controlled robot pipeline whose application is not constrained to a specific dataset or benchmark. (2) We build a novel VAR that provides reward signals to the downstream RL training. To our best knowledge, the VAR is the first representation that unifies the ASR, NLU, and the grounding module. (3) Our system exhibits promising results in multiple navigation and manipulation tasks. We demonstrate that our pipeline enables the robot to self-improve with limited amount of data from a new domain using both simulated and real-world experiments. (4) We create and solve the first AI environment that uses state-of-the-art free-form speech commands dataset for instruction-following tasks.


%The results are comparable to \cite{chang2020robot} that has access to numerous one-hot labels and carefully engineered rewards. 
 


 % The Kinova Gen3 policy was successfully transferred to a real-world Kinova Gen3 without training on real-world data.

%This paper is organized as follows: we review related works in Section~\ref{sec:related}.
%In Section~\ref{sec:methods}, we introduce our pipeline. We discuss simulated and real-world experiments in Section~\ref{sec:exp} and Section~\ref{sec:real_exp}, respectively. We conclude the paper in Section~\ref{sec:conclusion}.


